Sample Complexity of Power System State Estimation using Matrix Completion

In this paper, we propose an analytical framework to quantify the amount of data samples needed to obtain accurate state estimation in a power system - a problem known as sample complexity analysis in computer science. Motivated by the increasing adoption of distributed energy resources into the distribution-level grids, it becomes imperative to estimate the state of distribution grids in order to ensure stable operation. Traditional power system state estimation techniques mainly focus on the transmission network which involve solving an overdetermined system and eliminating bad data. However, distribution networks are typically underdetermined due to the large number of connection points and high cost of pervasive installation of measurement devices. In this paper, we consider the recently proposed state-estimation method for underdetermined systems that is based on matrix completion. In particular, a constrained matrix completion algorithm was proposed, wherein the standard matrix completion problem is augmented with additional equality constraints representing the physics (namely power-flow constraints). We analyze the sample complexity of this general method by proving an upper bound on the sample complexity that depends directly on the properties of these constraints that can lower number of needed samples as compared to the unconstrained problem. To demonstrate the improvement that the constraints add to distribution state estimation, we test the method on a 141-bus distribution network case study and compare it to the traditional least squares minimization state estimation method.

==> sections/archived_sections/approx_method_with_a.tex <==


In this section, we formulate an improved result on sample complexity that takes advantage of the linear equality constraints in the problem formulation.
The main challenge is on how to measure the information from the added constraints in terms of sample size which can be used to partially replace the need for extra measurements.
The intuition behind the usefulness of the added constraints \eqref{eq:min_rank_prob_const} is that each constraint may eliminate a single degree of freedom from the feasible solution set.
Thus, a set of constraints may decrease the search space for an approximation method so that less samples are needed to recover the underlying matrix $\mathbf{M}$.

\subsection{Degrees of Freedom in a Matrix} \label{sec:degrees}
Let $\mathbf{M}$ be an $n_1\times n_2$ matrix of rank $r$ which satisfies:
\begin{subequations}
	\begin{align}
		\mathbf{M} & = \sum_{k=1}^r\sigma_k\mathbf{u}_k\mathbf{v}_k^\intercal \label{eq:svd} \\
        \langle \mathbf{A}^{(l)}, \mathbf{M} \rangle & = b^{(l)} \quad \forall l\in\{1,\dots,\fixes{h}\} \label{eq:svd_const}
	\end{align}
\end{subequations}
where \eqref{eq:svd} is its Singular Value Decomposition (SVD).
Without loss of generality, we assume that $n_1\geq n_2$.
The vectors $\mathbf{u}_1,\dots,\mathbf{u}_r$ are unit vectors of size $n_1$ that are orthogonal to each other and the vectors $\mathbf{v}_1,\dots,\mathbf{v}_r$ are unit vectors of size $n_2$ that are orthogonal to each other.
The scalars $\sigma_1,\dots,\sigma_r$ which are used to linearly combine the matrices $\mathbf{u}_1\mathbf{v}_1^\intercal,\dots,\mathbf{u}_r\mathbf{v}_r^\intercal$ to be equal to $\mathbf{M}$ are called its singular values.
By convention, the singular values are listed in decreasing order so that $\sigma_k$ refers to the $k$th largest singular value in \eqref{eq:svd}.


The number of degrees of freedom of any $n_1\times n_2$ matrix of rank $r$ is $r(n_1+n_2-r)$.
This can be calculated by summing the degrees of freedom from each set individually that together make up the SVD \eqref{eq:svd}: $\{\mathbf{u}_1,\dots,\mathbf{u}_r\}$, $\{\mathbf{v}_1,\dots,\mathbf{v}_r\}$, and $\{\sigma_1,\dots,\sigma_r\}$.
The first and second sets have $r(n_1-1)-\sum_{k=1}^{r-1} k = r\left(n_1-\frac{1}{2}(r-1)\right)$ and $r\left(n_2-\frac{1}{2}(r-1)\right)$ degrees of freedom, respectively, since there are $r$ unit vectors of size $n_1$ (and $n_2$) while subtracting off the fact that the vectors within the set must be orthogonal to each other.
The last set trivially has $r$ degrees of freedom and summed all together it gives $r(n_1+n_2-r)$.


\subsection{High-Probability Exact Completion}

Due to the probabilistic nature of the question on sample complexity, the answer will also be probabilistic.
This is because for any given number of samples taken that is less than $(n_1-1)n_2$, there is some probability that the sampled locations will miss an entire row and thus have no information that can be used to recover it.
Thus, our goal will be to determine how large does $m$, the cardinality of $\Omega$, need to be to ensure a high probability of exact completion using the optimal solution to Problem \eqref{eq:nuc_norm_prob}.
Another way to frame the objective is to find the conditions on $m$ and $\mathbf{M}$ such that $\mathbf{M}$ is the unique solution to \eqref{eq:nuc_norm_prob} with some probability.


%%%% Coherence definition and Assumption
A property of the underlying matrix $\mathbf{M}$ that must be understood is how well its information is spread among its columns and rows.
A matrix with its information not well spread will require many samples.
For example, suppose there is a rank-1 matrix where $\mathbf{u}_1=[1 \ 0 \ \dots \ 0]^\intercal$ and $\mathbf{v}_1=[1 \ 0 \ \dots \ 0]^\intercal$ in \eqref{eq:svd}.
Therefore, in order to have a high probability of exact completion by any method, there must be a high probability that the location $(1,1)$ is in $\Omega$.
Otherwise, it would be impossible to have a guaranteed correct guess of the value in $(1,1)$ without having observed it.
For this reason, \cite{candes2009exact} defines a property on the space spanned by either $(\mathbf{u}_1,\dots,\mathbf{u}_r)$ or $(\mathbf{v}_1,\dots,\mathbf{v}_r)$ which measures the spread of the weight of its elements compared to the standard basis, called \emph{coherence}. 
\begin{definition}
	For any subspace $\mathcal{U}$ in $\mathbb{R}^n$ with dimension $r$, let the coherence of $\mathcal{U}$ be defined as
    \begin{align}
    	\mu(\mathcal{U}):=\frac{n}{r}\max_{i\in\{1,\dots,n\}} \left\|\mathbf{P}_\mathcal{U}\mathbf{e}_i\right\|^2 \nonumber
    \end{align}
    where $\mathbf{P}_\mathcal{U}$ is the orthogonal projection matrix onto $\mathcal{U}$ and $\mathbf{e}_i$ is the $i$-th standard basis vector with dimension $n$.
\end{definition}
The maximum possible value of $\mu(\mathcal{U})$ is $\frac{n}{r}$ when the subspace contains a standard basis vector, while its minimum possible value is 1, for example if its basis is spanned by vectors with elements that each have a magnitude of $\frac{1}{\sqrt{n}}$.
With the following assumption, the lack of spread of information within $\mathbf{M}$ can be bounded by bounding the coherence of the spaces defined by the vectors in its SVD \eqref{eq:svd}.
\begin{assumption}
    \label{ass:coherence}
	The coherence of $\mathcal{U}:=\text{span}(\mathbf{u}_1,\dots,\mathbf{u}_r)$ and the coherence of $\mathcal{V}:=\text{span}(\mathbf{v}_1,\dots,\mathbf{v}_r)$ are both upper bounded by some constant $\mu_0>0$, i.e.
    \begin{align}
    	\max\{\mu(\mathcal{U}),\mu(\mathcal{V})\}\leq \mu_0 \nonumber
    \end{align}
\end{assumption}

%%%% Assumption from maximum value of E

\fixes{To limit the concentration of information in the subgradient of the nuclear norm at $\mathbf{M}$ for any specific matrix location, an assumption is placed on the maximum value of sum of the rank-1 matrices $\mathbf{u}_1\mathbf{v}_1^\intercal,\dots,\mathbf{u}_r\mathbf{v}_r^\intercal$ through the parameter $\nu_0$.
\begin{assumption}
    \label{ass:maxEval}
	The absolute value of each element in $\sum_{k=1}^r\mathbf{u}_k\mathbf{v}_k^\intercal$ is upper bounded by $\nu_0\sqrt{r/(n_1n_2)}$.
\end{assumption}}

%%%% Vector space T
One important item needed in proving that $\mathbf{M}$ is the unique solution to \eqref{eq:nuc_norm_prob} is a vector space of matrices $\mathcal{T}$ that contains all $n_1\times n_2$ matrices which have a column space in $\mathcal{U}:=\text{span}(\mathbf{u}_1,\dots,\mathbf{u}_r)$, i.e. the column space of $\mathbf{M}$, and all $n_1\times n_2$ matrices which have a row space in $\mathcal{V}:=\text{span}(\mathbf{v}_1,\dots,\mathbf{v}_r)$, i.e. the row space of $\mathbf{M}$.
Specifically, a vector space $\mathcal{T}$ of matrices is built from all the combinations of $\mathbf{u}_1,\dots,\mathbf{u}_r$ that can span the column space and all the combinations of $\mathbf{v}_1,\dots,\mathbf{v}_r$ that can span the row space via their outer products with the vectors $\{\mathbf{x}_1,\dots,\mathbf{x}_r\}\in\mathbb{R}^{n_2}$ and $\{\mathbf{y}_1,\dots,\mathbf{y}_r\}\in\mathbb{R}^{n_1}$:
\begin{align}
    \mathcal{T}:=\bigg\{\sum_{k=1}^r\left(\mathbf{u}_k\mathbf{x}^\intercal_k+\mathbf{y}_k\mathbf{v}_k^\intercal\right):\mathbf{x}_k\in\mathbb{R}^{n_2},\mathbf{y}_k\in\mathbb{R}^{n_1}\bigg\} \nonumber
\end{align}
This vector space has a dimension of $r(n_1+n_2-r)$ which is equal to the degrees of freedom in any $n_1\times n_2$ matrix of rank $r$ (see Section \ref{sec:degrees}). 
Additionally, its orthogonal complement $\mathcal{T}^\perp$ will  also be important which is the vector space that contains the matrices $\mathbf{y}\mathbf{x}^\intercal$, where $\mathbf{y}$ is any vector orthogonal to the column space of $\mathbf{M}$ and $\mathbf{x}$ is any vector orthogonal to the row space of $\mathbf{M}$.


Conditions on the orthogonal projection of the nuclear norm's subgradient onto $\mathcal{T}$ and $\mathcal{T}^\perp$ will be shown later to give sufficient conditions for determining if a particular matrix is optimal to Problem \eqref{eq:nuc_norm_prob} (see Lemma \ref{thm:nuc_norm_opt}).
The orthogonal projection of $\mathbf{X}\in\mathbb{R}^{n_1\times n_2}$ onto $\mathcal{T}$ can be stated from
its projections onto $\mathcal{U}$ and $\mathcal{V}$ (see Equation (3.5) in~\cite{candes2009exact}):
\begin{align}
    \mathcal{P}_\mathcal{T}(\mathbf{X}) = \mathbf{P}_\mathcal{U}\mathbf{X} + \mathbf{X}\mathbf{P}_\mathcal{V} - \mathbf{P}_\mathcal{U}\mathbf{X}\mathbf{P}_\mathcal{V} \label{eq:PT_defn}
\end{align}
where $\mathbf{P}_\mathcal{U}$ and $\mathbf{P}_\mathcal{V}$ are the orthogonal projection matrices onto $\mathcal{U}$ and $\mathcal{V}$ respectively.
The orthogonal projection onto $\mathcal{T}^\perp$ can also be stated in the same manner:
\begin{align}
    \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{X}) = (\mathbf{I}_{n_1}-\mathbf{P}_\mathcal{U})\mathbf{X}(\mathbf{I}_{n_2}-\mathbf{P}_\mathcal{V}). \nonumber
\end{align}


%%%% Information from equality constraints
\fixes{To measure the amount of useful information held in the linear equalities \eqref{eq:svd_const} that can explain $\mathbf{M}$, we develop quantities similar to the upper bounds of Assumptions \ref{ass:coherence} and \ref{ass:maxEval} for the vector space spanned by $\mathbf{A}^{(1)},\dots,\mathbf{A}^{(\fixes{h})}$, denoted by $\mathcal{Q}$.
First, we measure how much of the vector space $\mathcal{T}$ is covered and how much remains uncovered by $\mathcal{Q}$ with $\mu_\mathcal{Q}$ and $\mu_{\mathcal{Q}^\perp}$, respectively:
\begin{subequations}
    \begin{align}
        \mu_\mathcal{Q} & := \frac{1}{n_1n_2}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\left\|\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}\left(\mathbf{e}_i\mathbf{e}_j^\intercal\right)\right\|_F^2 \\
        \mu_{\mathcal{Q}^\perp} & := \frac{1}{n_1n_2}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\left\|\mathcal{P}_\mathcal{T}\mathcal{P}_{\mathcal{Q}^\perp}\left(\mathbf{e}_i\mathbf{e}_j^\intercal\right)\right\|_F^2.
    \end{align}
\end{subequations}
These measures give an element-wise average of coverage or non-coverage by $\mathcal{Q}$ in $\mathcal{T}$ which are each upper bounded by 1.
Second, we measure how much of the subgradient of the nuclear norm at $\mathbf{M}$ is contained or not contained in $\mathcal{Q}$ with $\nu_\mathcal{Q}$ and $\nu_{\mathcal{Q}^\perp}$, respectively:
\begin{subequations}
    \begin{align}
        \nu_\mathcal{Q} & := \frac{1}{r}\left\|\mathcal{P}_\mathcal{Q}\left(\mathbf{E}\right)\right\|_F^2 \\
        \nu_{\mathcal{Q}^\perp} & := \frac{1}{r}\left\|\mathcal{P}_{\mathcal{Q}^\perp}\left(\mathbf{E}\right)\right\|_F^2.
    \end{align}
\end{subequations}
where $\mathbf{E}:=\sum_{k=1}^r\mathbf{u}_k\mathbf{v}_k^\intercal$ and each has a maximum value of 1.}

\fixes{Notice that if $\mathcal{Q}$ covers the entire space of $\mathcal{T}$ (i.e. $\mathcal{Q}\supseteq\mathcal{T}$), then $\mu_{\mathcal{Q}^\perp}=\nu_{\mathcal{Q}^\perp}=0$ since $\mathbf{E}\in\mathcal{T}$.
On the other hand, if $\mathcal{Q}$ does not cover any of the space of $\mathcal{T}$ (i.e. $\mathcal{Q}^\perp\supseteq\mathcal{T}$), then $\mu_\mathcal{Q}=\nu_\mathcal{Q}=0$.
These two extreme cases will be important in explaining the significance of our main result, Theorem \ref{thm:samp_complex}, in regards to how much fewer samples are needed for exact completion.}

% OLD
%%%% Assumption from equality constraints
%To measure the amount of information held in the linear equalities \eqref{eq:svd_const} that can explain $\mathbf{M}$, we develop a quantity similar to coherence.
%Instead of trying to measure the spread of information as in coherence, we are focused on how much useful information from linear equality matrices $\mathbf{A}^{(1)},\dots,\mathbf{A}^{(\fixes{h})}$ can replace that of the rank-1 matrices $\mathbf{u}_1\mathbf{v}_1^\intercal,\dots,\mathbf{u}_r\mathbf{v}_r^\intercal$.
%Useful information from a matrix $\mathbf{A}^{(l)}$ is determined as its projection onto $\mathcal{T}$ since that is the space which contains $\mathbf{M}$.
%From these ideas, we have the following assumption which bounds how much of the rank-1 matrices remain uncovered by a linear combination of the useful information in $\mathbf{A}^{(1)},\dots,\mathbf{A}^{(\fixes{h})}$ in terms of number of elements in $\mathbf{M}$.
%\begin{assumption}
%    \label{ass:equality}
%	There exists a vector $\boldsymbol{\gamma}\in\mathbb{R}^\fixes{h}$ and a constant $\mu_A$ such that
%	\begin{subequations}
%	\label{eq:equality_assump}
%    \begin{align}
%    	\frac{n_1n_2}{r}\left\| \mathbf{F} \right\|_F^2  \leq \mu_A \label{eq:constr_bound}
%    \end{align}
%    where 
%    \begin{align}
%        \mathbf{F}:= \sum_{k=1}^r\mathbf{u}_k\mathbf{v}_k^\intercal + \sum_{l=1}^{\fixes{h}} \gamma_l\mathcal{P}_\mathcal{T}\left(\mathbf{A}^{(l)}\right). \label{eq:F_defn}
%    \end{align}
%    \end{subequations}
%\end{assumption}
%A $\mu_A$ of a certain value means that the equivalent information of $n_1n_2-\mu_A$ observations are encoded in the linear equality constraints for specifying the $r$ rank-1 matrices.
%By minimizing the LHS of \eqref{eq:constr_bound} w.r.t. $\boldsymbol{\gamma}$, one could find the minimum value of $\mu_A$ which corresponds to the most amount of information.
%Note that $\left\| \sum_{k=1}^r\mathbf{u}_k\mathbf{v}_k^\intercal \right\|_F^2 = r$.
%Hence, the upper bound on the minimum value of $\mu_A$ is $n_1n_2$ when either $\boldsymbol{\gamma}=\mathbf{0}$ or none of the equality constraints has useful information, i.e. $\mathcal{P}_\mathcal{T}\left(\mathbf{A}^{(l)}\right)=\mathbf{0}:\forall l\in\{1,\dots,\fixes{h}\}$.
%The lower bound on the minimum value of $\mu_A$ is 0 when the useful information in equality constraints can completely replace those from the SVD vectors.
%However, a $\mu_A$ of 0 does not mean that no observations are needed because the useful information described above only refers to the information in the $r$ rank-1 matrices but does not say anything about the singular values themselves that need to be determined.


%%%% Sample Complexity Theorem
Finally, using the above definitions and assumptions, we can state our theorem on sample complexity with a high-probability matrix completion guarantee. 

\begin{theorem}
    \label{thm:samp_complex}
    Let $\mathbf{M}$ be an $n_1 \times n_2$ matrix with $n_1 \geq n_2$ such that the following $\fixes{h}$ linear equality constraints are satisfied: $\langle \mathbf{A}^{(l)}, \mathbf{M} \rangle = b^{(l)}$ for all $l\in\{1,\dots,\fixes{h}\}$.
    Also, let $\mathbf{M}$ be of rank $r$ and have the following singular value decomposition $\sum_{k=1}^r\sigma_k\mathbf{u}_k\mathbf{v}_k^\intercal$ that satisfies Assumptions \ref{ass:coherence} and \ref{ass:equality}.
    Suppose that $m$ entries of $\mathbf{M}$ are sampled uniformly at random. Then there exists a constant $C$ such that if 
    \begin{align}
        m > \max \left\{6 \mu_A, C\mu_0\beta n_1\log n_1 \right\}r \label{eq:thm_samp_complex}
    \end{align}
    for some $\beta>1$, then the solution to Problem \eqref{eq:nuc_norm_prob} is unique and equal to $\mathbf{M}$ with probability at least $1-6n_1^{-\beta}$.
\end{theorem}

The proof is given in detail in the next subsection.

\begin{remark}
    If $\boldsymbol{\gamma}$ is set to $\mathbf{0}$ in \eqref{eq:F_defn}, then the sample complexity proof of the unconstrained matrix completion problem in \cite{candes2009exact} follows directly.
    Therefore, a new sample complexity bound for the constrained matrix completion problem can be taken as the minimum between the bound in Theorem \ref{thm:samp_complex} and Theorem 1.3 in \cite{candes2009exact} by either minimizing the LHS of \eqref{eq:constr_bound} or setting $\boldsymbol{\gamma}$ to $\mathbf{0}$, respectively.
    This is especially useful for the case when $\mu_A\geq \frac{n_1n_2}{6}$, since the RHS of \eqref{eq:thm_samp_complex} would become greater than $n_1n_2$.
\end{remark}

This theorem shows us that the constraints can decrease the number of samples needed down to a certain point.
With no constraints, $\mu_A$ is equal to $n_1n_2$.
But as constraints with useful information are added, the value of $6\mu_A$ decreases until it becomes equal to $C\mu_0\beta n_1\log n_1$ where the lack of information spread within $\mathbf{M}$ becomes the dominating factor.

When connecting this theoretical result back to the state estimation problem for a distribution network, $n_1$ represents the number of buses and lines; see Section \ref{sec:state_est_prob}.
As the size of the distribution network grows, then  the number of samples needed to estimate the state with high probability will at best increase linearly with $n_1$ via $\mu_A$ in \eqref{eq:equality_assump} or at worst $n_1\log n_1$.


\subsection{Proof of Theorem \ref{thm:samp_complex}}

%%%% Bernoulli Sampling
A challenge with the uniform random sampling model is that the probability that an element will be sampled depends on which ones have already been sampled.
Instead of proving Theorem \ref{thm:samp_complex} directly with uniform random sampling, we prove it with the following Bernoulli sampling model:
\begin{subequations}
    \label{eq:bernoulli}
    \begin{align}
        \mathbb{P}(\delta_{ij}=1) & = p := \frac{m}{n_1n_2} \\
        \Omega' & := \left\{(i,j):\delta_{ij}=1\right\}.
    \end{align}
\end{subequations}
since the probability an element will be sampled is independent of whether any other element has been sampled or not.
Then we can invoke the result from \cite{candes2006robust}, Section II.C, which states that the probability of failure with the uniform sampling model can be bounded by twice that of the Bernoulli sampling model.

%%%% Nuclear Norm Problem Sufficient conditions
First, we have a lemma which states sufficient optimality conditions for Problem \eqref{eq:nuc_norm_prob} which are later shown in the proof to be satisfied by $\mathbf{M}$ under certain probabilistic conditions.
The two lemmas following the first are used in the proof to define the conditions which $\mathbf{M}$ satisfies Lemma \ref{thm:nuc_norm_opt}.
Let $\mathcal{P}_\Omega(\mathbf{X})$ be the projection operator onto $\Omega$ where projection's element equals $X_{ij}$ if $(i,j)\in\Omega$ or 0 otherwise.
Also, let the $\mathcal{R}_\Omega(\mathbf{X})$ be the sampling operator which maps the elements of $\mathbf{X}$ to a vector of size $m$ for only the element locations that are in $\Omega$.
%\fixes{and let $\mathcal{R}_\mathcal{Q}(\mathbf{X})$ be the constraint operator which maps $\mathbf{X}$ to a vector of size $h$ such that the $l$-th element is equal to $\langle\mathbf{A}^{(l)},\mathbf{X}\rangle$.}

\begin{lemma}
    \label{thm:nuc_norm_opt}
    Suppose that there exists some matrix $\mathbf{X}_0=\sum_{k=1}^{r}\sigma_k\mathbf{u}_k\mathbf{v}_k^\intercal$ of rank $r$ that is feasible to Problem \eqref{eq:nuc_norm_prob}.
    If it satisfies the two following conditions:
    \begin{enumerate}
        \item There exists a dual point $(\boldsymbol{\lambda},\boldsymbol{\gamma})$ where $\mathbf{Y}=\mathcal{R}_\Omega^\intercal\boldsymbol{\lambda}+\sum_{l=1}^{\fixes{h}} \gamma_l\mathbf{A}^{(l)}$ such that
        \begin{subequations}
            \begin{align}
                \mathcal{P}_\mathcal{T}(\mathbf{Y}) & = \sum_{k=1}^{r}\mathbf{u}_k\mathbf{v}_k^\intercal \\
                \left\|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y})\right\| & < 1
            \end{align}
        \end{subequations}
        \item The sampling operator $\mathcal{R}_\Omega$ restricted to the elements of $\mathcal{T}$ is injective.
    \end{enumerate}
    then $\mathbf{X}_0$ is the unique solution to Problem \eqref{eq:nuc_norm_prob}.
\end{lemma}
See Appendix \ref{sec:proof_nuc_norm_opt} for the proof.

%%%% Bound norm to show that inverse exists

\begin{lemma}
    \label{thm:bound_frob_OmegaT}
    Suppose that if $\Omega$ is sampled according to the Bernoulli model \eqref{eq:bernoulli}, $n_1\geq n_2$, and Assumption \ref{ass:coherence} is satisfied, then there is a numerical constant $C_R$ such that for all $\beta>1$,
    \begin{align}
        \left\|\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}(\mathbf{X})\right\|_F \leq \sqrt{\frac{3p}{2}}\left\|\mathcal{P}_\mathcal{T}(\mathbf{X})\right\|_F
    \end{align}
    with probability at least $1-3n_1^{-\beta}$ provided that $C_R \sqrt{\frac{\mu_0\beta rn_1\log n_1}{m}}\leq\frac{1}{2}$.
\end{lemma}
See Corollary 4.3 in \cite{candes2009exact} for the proof.


%%%% Bound the Spectral Norm of sum H^k

\begin{lemma}
    \label{thm:bound_Hsum}
    Suppose that if $\Omega$ is sampled according to the Bernoulli model \eqref{eq:bernoulli}, $n_1\geq n_2$, and Assumptions \ref{ass:coherence} and \ref{ass:equality} are satisfied, then there are numerical constants $C_R$ and $C_{k_0}$ such that for all $\beta>1$,
    \begin{align}
        \frac{1}{p}\left\|\left(\mathcal{P}_{\mathcal{T}^\perp}\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}\right)\sum_{k=k_0}^\infty \mathcal{H}^k(\mathbf{F})\right\| \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber \\
        \leq  \sqrt{\frac{6\mu_A r}{m}} \left(\frac{C_R^2\mu_0\beta rn_1\log n_1}{m}\right)^{k_0/2} \label{eq:spectral_norm_sum}
    \end{align}
    with probability at least $1-3n_1^{-\beta}$ provided that $m\geq 4C_R^2\mu_0\beta rn_1\log n_1$.
    The operator $\mathcal{H}$ is defined by \eqref{eq:H_defn}.
\end{lemma}
See Appendix \ref{sec:proof_bound_Hsum} for the proof.


Finally with the above lemmas in place, we formally prove Theorem \ref{thm:samp_complex}.
The main effort of this proof will be to show that there exists a subgradient of the nuclear norm at $\mathbf{M}$, the underlying matrix, which satisfies Lemma \ref{thm:nuc_norm_opt} under high-probability given a sufficient number of samples.
If Lemma \ref{thm:nuc_norm_opt} is satisfied, then the optimal solution to Problem \eqref{eq:nuc_norm_prob} and $\mathbf{M}$ uniquely coincide.
It is first proved for the Bernoulli sampling model \eqref{eq:bernoulli} and then the results are converted into that of being under the uniform sampling model.
\begin{proof}
    %%%% Derivation of candidate Y
    The first step is to find a candidate $\mathbf{Y}$ that satisfies the first condition of Lemma \ref{thm:nuc_norm_opt} by solving
    \begin{subequations}
        \label{eq:candidateY_prob}
	    \begin{align}
		    \min_{\mathbf{X},\fixes{\mathbf{Z}}} \quad & \frac{1}{2}\|\mathbf{X}\|_F^2\fixes{+\frac{1}{2a}\|\mathbf{Z}\|_F^2} \\
    	    \text{s.t.} \quad &  \mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega(\mathbf{X}) \fixes{+\mathcal{P}_\mathcal{Q}(\mathbf{Z})}\right)= \fixes{\mathbf{E}}
	    \end{align}
    \end{subequations}
    \fixes{where $a>0$ can later be tuned} and using its solution \fixes{$\mathbf{X}+\mathbf{Z}$} as $\mathbf{Y}$.

    The Karush-Kuhn-Tucker conditions for optimality with dual matrix $\boldsymbol{\nu}$ \fixes{(not to be confused with the constants $\nu_0$, $\nu_\mathcal{Q}$, and $\nu_{\mathcal{Q}^\perp}$)} gives us
    \begin{subequations}
        \begin{align}
            \mathbf{X} - \mathcal{P}_\Omega\mathcal{P}_\mathcal{T}(\boldsymbol{\nu}) & = 0 \label{eq:candidateY_prob_kkt1} \\
            \fixes{\frac{1}{a}\mathbf{Z} - \mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{T}(\boldsymbol{\nu})} & = 0 \label{eq:candidateY_prob_kkt2} \\
            \mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega(\mathbf{X}) \fixes{+\mathcal{P}_\mathcal{Q}(\mathbf{Z})}\right) - \fixes{\mathbf{E}} & = 0. \label{eq:candidateY_prob_kkt3}
        \end{align}
    \end{subequations}
    To solve for a closed form of $\mathbf{X}\fixes{+\mathbf{Z}}$, start with \eqref{eq:candidateY_prob_kkt1} \fixes{and \eqref{eq:candidateY_prob_kkt2}:}
    \begin{subequations}
        \begin{align}
            \mathbf{X} & = \mathcal{P}_\Omega\mathcal{P}_\mathcal{T}(\boldsymbol{\nu}), \label{eq:candidateY_prob_X}  \\
            \fixes{\mathbf{Z}} & = \fixes{a\mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{T}(\boldsymbol{\nu})}. \label{eq:candidateY_prob_Z}
    \end{align}
    \end{subequations}
    Next, apply $\mathcal{P}_\mathcal{T}\mathcal{P}_\Omega$ \fixes{and $\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}$, respectively:}
    \begin{align}
        \mathcal{P}_\mathcal{T}\mathcal{P}_\Omega(\mathbf{X}) & = \mathcal{P}_\mathcal{T}\mathcal{P}_\Omega\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}(\boldsymbol{\nu}) = \mathcal{P}_\mathcal{T}\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}(\boldsymbol{\nu}), \nonumber \\
        \fixes{\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{Z})} & = \fixes{a\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{T}(\boldsymbol{\nu}) = a\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{T}(\boldsymbol{\nu}),} \nonumber
    \end{align}
    and then apply \eqref{eq:candidateY_prob_kkt3} \fixes{after summing the two} to get
    \begin{align}
        \fixes{\mathbf{E}} = \mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega\fixes{+a\mathcal{P}_\mathcal{Q}}\right)\mathcal{P}_\mathcal{T}(\boldsymbol{\nu}). \nonumber
    \end{align}
    Taking the inverse, assuming it exists, gives
    \begin{align}
        \boldsymbol{\nu} = \left(\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega\fixes{+a\mathcal{P}_\mathcal{Q}}\right)\mathcal{P}_\mathcal{T}\right)^{-1}(\fixes{\mathbf{E}}), \nonumber
    \end{align}
    and finally applying it to \fixes{\eqref{eq:candidateY_prob_X} and \eqref{eq:candidateY_prob_Z}} gives the candidate $\mathbf{Y}$:
    \begin{align}
        \mathbf{Y} & = \mathbf{X}\fixes{+\mathbf{Z}} \nonumber \\
        & = \left(\mathcal{P}_\Omega\fixes{+a\mathcal{P}_\mathcal{Q}}\right)\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega\fixes{+a\mathcal{P}_\mathcal{Q}}\right)\mathcal{P}_\mathcal{T}\right)^{-1}(\fixes{\mathbf{E}}). \label{eq:candidateY}
    \end{align}

    The benefit to the formulation of Problem \eqref{eq:candidateY_prob} is that it minimizes $\|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y})\|_F$.
    By Pythagoras we have
    \begin{align}
        \|\mathbf{Y}\|_F^2 & = \|\mathcal{P}_{\mathcal{T}}(\fixes{\mathbf{X}+\mathbf{Z}})\|_F^2 + \|\mathcal{P}_{\mathcal{T}^\perp}(\fixes{\mathbf{X}+\mathbf{Z}})\|_F^2. \nonumber
    \end{align}
    The first term on the RHS remains constant since $\mathcal{P}_\mathcal{T}(\fixes{\mathbf{X}+\mathbf{Z}})=\mathcal{P}_\mathcal{T}\left(\fixes{\mathcal{P}_\Omega(\mathbf{X}) +\mathcal{P}_\mathcal{Q}(\mathbf{Z})}\right)=\fixes{\mathbf{E}}$ since \fixes{from \eqref{eq:candidateY_prob_X} and \eqref{eq:candidateY_prob_Z} we have $\mathcal{P}_\Omega(\mathbf{X})=\mathcal{P}_\Omega\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}(\boldsymbol{\nu})=\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}(\boldsymbol{\nu})=\mathbf{X}$ and $\mathcal{P}_\mathcal{Q}(\mathbf{Z})=\mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{T}(\boldsymbol{\nu})=\mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{T}(\boldsymbol{\nu})=\mathbf{Z}$, respectively.}
    Thus, only the second term can vary  which is an upper bound on the spectral norm $\left\|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y})\right\|$.

    The next step is to transform the candidate subgradient $\mathbf{Y}$ given by Equation \eqref{eq:candidateY} into a more manageable form.
    Notice that by taking its projection onto $\mathcal{T}$, the candidate $\mathbf{Y}$ trivially satisfies the first part of the first condition of Lemma \ref{thm:nuc_norm_opt}.
    
    \fixes{To express $\left(\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega\fixes{+a\mathcal{P}_\mathcal{Q}}\right)\mathcal{P}_\mathcal{T}\right)^{-1}(\mathbf{E})$ in an analyzable form via the Neumann series,} let us define the following operator
    \begin{align}
        \mathcal{H} := \mathcal{P}_\mathcal{T}-\frac{1}{p\fixes{+q}}\mathcal{P}_{\mathcal{T}}\left(\mathcal{P}_\Omega\fixes{+a\mathcal{P}_\mathcal{Q}}\right)\mathcal{P}_\mathcal{T} \label{eq:H_defn}
    \end{align}
    \fixes{where $q\in[0,1]$ is an adjustable parameter,} which gives
    \begin{align}
        \left(\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega\fixes{+a\mathcal{P}_\mathcal{Q}}\right)\mathcal{P}_\mathcal{T}\right)^{-1}(\fixes{\mathbf{E}}) & = ((p\fixes{+q})(\mathbf{I}-\mathcal{H}))^{-1}(\fixes{\mathbf{E}}) \nonumber \\
        & = \frac{1}{p\fixes{+q}}\sum_{k=0}^\infty \mathcal{H}^k(\fixes{\mathbf{E}}). \nonumber
    \end{align}
    From Lemma \ref{thm:bound_opnormH}, we have the assumption that $\|\mathcal{H}\|<1$, which means that the Neumann series converges in the operator norm.
    This results in $\frac{1}{p}\mathcal{P}_\mathcal{T}\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}$ being invertible.
    Since it is invertible, then it must mean that $\mathcal{P}_\Omega$ is injective restricted to elements in $\mathcal{T}$ which satisfies the second condition of Lemma \ref{thm:nuc_norm_opt} with regards to the sampling operator $\mathcal{R}_\Omega$.
    
    From the above Neumann series and since $\mathbf{F}$ is in $\mathcal{T}$, we can express $\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y})$ as
    \begin{align}
        \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y}) = \frac{1}{p}\left(\mathcal{P}_{\mathcal{T}^\perp}\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}\right)\left(\sum_{k=0}^\infty \mathcal{H}^k(\mathbf{F})\right). \nonumber
    \end{align}
    Lemma \ref{thm:bound_Hsum} can now be used by bounding its RHS of \eqref{eq:spectral_norm_sum} to be less than 1 as a condition to satisfy the second part of the first condition of Lemma \ref{thm:nuc_norm_opt} which results in
    \begin{align}
        \sqrt{\frac{6\mu_A r}{m}} \left(\frac{C_R^2\mu_0\beta rn_1\log n_1}{m}\right)^{k_0/2} < 1 \nonumber
    \end{align}
    Then solving for $m$ gives
    \begin{align}
        m > \left(6\mu_A r\right)^{1/(k_0+1)} \left(C_R^2\mu_0\beta rn_1\log n_1\right)^{k_0/(k_0+1)}. \nonumber 
    \end{align}
    Setting $k_0=0$ so that the LHS of \eqref{eq:spectral_norm_sum} equals $\left\|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y})\right\|$ and making sure to satisfy Lemma \ref{thm:bound_Hsum}'s condition on $m$ for gives
    \begin{align}
        m > \max \left\{6\mu_A r, 4C_R^2\mu_0\beta rn_1\log n_1 \right\}. \nonumber
    \end{align}
    Setting $C:=4C_R^2$ gets the form in the theorem's statement.
    
    However, everything previous to this point proves the satisfaction of Lemma \ref{thm:nuc_norm_opt} for the Bernoulli sampling model with probability at least $1-3n_1^{-\beta}$ as stated in Lemmas \ref{thm:bound_opnormH} and \ref{thm:bound_Hsum}.
    From \cite{candes2006robust} Section II.C, the probability of failure with the uniform sampling model can be bounded by twice that of the Bernoulli sampling model.
    Therefore, we multiply the failure probability by two to get $1-6n_1^{-\beta}$ as stated in the theorem.
\end{proof}

==> sections/archived_sections/perf_evaluation_old.tex <==
\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/toy_sim02_samp_muA_vs_numconst.pdf}
    \caption{(Top) Minimum sample size for exact matrix completion with 95\% probability  vs. number of linear equality constraints.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints and solving it without constraints.
    (Bottom) Minimum value of $\mu_A$ for Assumption \ref{ass:equality} vs. number of linear equality constraints.}
    \label{fig:toy_sim02_samp_muA_vs_numconst}
\end{figure}


First, we demonstrate how the addition of linear equality constraints can decrease the number of samples needed to exactly recover the underlying matrix.
Afterwards, we apply the technique to distribution network data to show how estimation error can be decreased.

\subsection{Matrix Completion with Constraints}
\label{sec:perf_eval_toy}

The goal of this simulation is to observe the impact of the size of $\mu_A$ in Assumption \ref{ass:equality} on the sample complexity through randomly generated matrix completion examples.

\subsubsection{Setup}

%%%% Generating M
The underlying matrix $\mathbf{M}$ was built by first generating an $n_1\times n_2$ matrix with each element sampled independently from a standard normal distribution.
The singular value decomposition of the generated matrix was taken which gives $n_2$ singular values $(\sigma_1,\dots,\sigma_{n_2})$, assuming $n_1\geq n_2$, and their associated basis vectors $(\mathbf{u}_1,\dots,\mathbf{u}_{n_2})$ and $(\mathbf{v}_1,\dots,\mathbf{v}_{n_2})$.
To make the rank of $\mathbf{M}$ to be $r$, $r$ integers are chosen uniformly at random without replacement from 1 to $n_2$ which correspond to the index of the triplet $(\sigma_k,\mathbf{u}_k,\mathbf{v}_k)$.
The chosen triplets and are combined together in \eqref{eq:svd} to get the final $\mathbf{M}$ that is used in the simulation.

%%%% Generating A and b
The equality constraints \eqref{eq:svd_const} are generated in two steps.
First, each matrix $\mathbf{A}^{(l)}$ is made by generating an $n_1\times n_2$ matrix with each element sampled independently from a standard normal distribution.
Afterwards each vector $b^{(l)}$ is determined by evaluating the LHS of \eqref{eq:svd_const}.
There are $n_1n_2$ equality constraints generated by this process.
The $\mu_A$ calculated for a given set of constraints was calculated by minimizing the LHS of \eqref{eq:constr_bound}.

%%%% Generating the uniform sampling
The uniform sampling was done by taking a random permutation of all the locations for an $n_1\times n_2$ matrix and using the first $m$ locations as the observed samples.
To increase (decrease) number of samples, the next (previous) locations in the permutation were simply added to (subtracted from) the existing observed samples.
Multiple random permutations were tested in parallel so that a sample probably of exact matrix completion could be calculated among them.
The probability of exact matrix completion for a given sample size was calculated as the fraction of random permutation sequences in which the solution to \eqref{eq:nuc_norm_prob} subtracted from $\mathbf{M}$ resulted in a Frobenius norm smaller that a specific tolerance.

%%%% Specifics
The specifics of this simulation were under the following settings: $n_1=40$, $n_2=5$, $r=2$, 100 random permutations, and the maximum tolerance in the Forbenius norm to determine exact completion was set to $10^{-5}$.

\subsubsection{Results}

%%%% Sample size vs. number of constraints
To demonstrate the sample complexity upper bound given by Theorem \ref{thm:samp_complex}, we fixed 
the probability for exact matrix completion for a given set of linear equality constraints to 95\%.
%Our aim was to demonstrate the sample complexity upper bound given by Theorem \ref{thm:samp_complex} by fixing the probability constraint to 95\% for exact matrix completion for a given set of linear equality constraints.
This was done by increasing the sample size until 95 out of the 100 randomly permuted sequences of matrix locations each gave an exact matrix completion.
The final sample size was recorded in top half of Figure \ref{fig:toy_sim02_samp_muA_vs_numconst} for each set of randomly generated constraints.
The constrained nuclear norm minimization matrix completion method \eqref{eq:nuc_norm_prob} was tested against its unconstrained version.
The figure shows that increasing the number of constraints decreases monotonically the number of samples needed to exactly complete a matrix for a given probability.
Interestingly without the constraints, it required a sample size of 190 which is 95\% of the matrix elements.
This shows the performance increase by taking advantage of constraints when they are available.

%%%% \mu_A vs. number of constraints
Additionally, the minimum value of $\mu_A$ from Assumption \ref{ass:equality} for a given set of constraints was plotted against the constraint set size in the bottom half of Figure \ref{fig:toy_sim02_samp_muA_vs_numconst}.
This shows that a decreasing $\mu_A$ trends with an increasing constraint set size and a decreasing sample size requirement.
Since each constraint matrix $\mathbf{A}^{(l)}$ can be assumed to be linearly independent, notice that $\mu_A$ reaches 0 with 86 constraints which is exactly $\text{dim}(\mathcal{T})=r(n_1+n_2-r)=86$.

%%%% Sample size vs. \mu_A
The data from Figure \ref{fig:toy_sim02_samp_muA_vs_numconst} were re-plotted in Figure \ref{fig:toy_sim02_samp_vs_muA} to show the sample size requirement vs. $\mu_A$.
This shows the approximate linear relationship between the sample complexity and $\mu_A$ which matches Theorem \ref{thm:samp_complex}.


\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/toy_sim02_samp_vs_muA.pdf}
    \caption{Minimum sample size for exact matrix completion with 95\% probability  vs. Minimum value of $\mu_A$ for Assumption \ref{ass:equality}.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints and solving it without constraints.}
    \label{fig:toy_sim02_samp_vs_muA}
\end{figure}



\subsection{Distribution Network}
\label{sec:perf_eval_distnet}

Using a power system emulator, our goal is to show how incorporating equality constraints based on the physics of the system can improve the accuracy for state estimation.

\subsubsection{Setup}

%%%% Data for matrix and constraints

The distribution network data was created using MATPOWER~\cite{zimmerman2011matpower} on a 141 bus radial distribution network test case~\cite{khodr2008maximum}.
A diagram of the network is shown in Appendix \ref{sec:app_dist}.
The underlying matrix $\mathbf{M}$ that represents the state of the power system was formed according to the structure described in Section \ref{sec:state_est_prob} with all quantities being transferred into pu.
Therefore, the state matrix $\mathbf{M}$ has 281 rows and 17 columns.
The set of $4(n_\text{b}+n_\text{l})=1124$ linear equality constraints \eqref{eq:nuc_norm_prob_const} were formed according to the following linear power system equations: \eqref{eq:syseqn_line_pwrcons}-\eqref{eq:syseqn_ohms_law}.
An additional set of $n_\text{l}=140$ linear equality constraints were formed according to the linear approximation equations \eqref{eq:lin_approx_const}.

%%%% Sampling

To sample the values of the state matrix $\mathbf{M}$, we set that Bus 1 and Bus 80 each have a PMU which can measure all 8 bus state values.
The remaining 139 buses and 140 lines were chosen uniformly at random to be measured.
When a bus was chosen, only the following 4 values were revealed: the real and reactive power injections, the magnitude of the voltage, and the magnitude of the current injection.
Therefore for both the voltage and current injections, the complex parts are never observed except for Buses 1 and 80 at the start.
When a line was chosen, only the following 5 values were revealed: real and reactive power injections into the line for both the From and To sides of the line, and the magnitude of the current flowing through the line.
Therefore, the real and reactive power losses and the complex current flow are never observed.
The number of samples in the figures refer to the number of lines and buses samples, not the number of data points taken.
For each sample size, 40 different random permutations of the buses and lines were used to do the uniform sampling, similar to Section \ref{sec:perf_eval_toy}.

%%%% Benchmarks

Two different sets of constraints were tested in Problem \eqref{eq:nuc_norm_prob} for state estimation.
The first set only includes the linear equality constraints derived from the linear power system model equations \eqref{eq:syseqn_line_pwrcons}-\eqref{eq:syseqn_ohms_law}.
The second set are the linear equality constraints derived from the linear approximation equations \eqref{eq:lin_approx_const}.
We run four different combinations of these constraint sets to estimate the state of the distribution network: first set alone (``w/ const"), second set alone (``w/ appx""), first and second set together (``w/ const+appx"), and no constraints (``none'').
To measure the estimation error, the Root Mean Squared Error (RMSE) was taken for each measurement type for the unmeasured values.
The final reported error value for each measurement type was the RMSE averaged among the random samples.


\begin{figure}[t]
    \subfigure[]{\includegraphics[width=0.95\columnwidth]{images/case141_sim03_bus_volterr_mag_vs_samp.pdf}\label{fig:case141_sim03_bus_volterr_mag_vs_samp}}
    %
    \subfigure[]{\includegraphics[width=0.95\columnwidth]{images/case141_sim03_bus_volterr_mag_cdf.pdf}\label{fig:case141_sim03_bus_volterr_mag_cdf}}
    %
    \caption{(a) Average RMSE for estimated voltage magnitude at unobserved buses vs. sample size which is the total number of buses and lines with observed state data.
    The circles represent where (b) is located in (a).
    (b) Cumulative Distribution Function of voltage magnitude estimation error at unmeasured buses given 140 bus/line measurement samples.}
\end{figure}

\begin{figure}[t]
    \subfigure[]{\includegraphics[width=0.95\columnwidth]{images/case141_sim03_bus_volterr_angle_vs_samp.pdf}\label{fig:case141_sim03_bus_volterr_angle_vs_samp}}
    %
    \subfigure[]{\includegraphics[width=0.95\columnwidth]{images/case141_sim03_bus_volterr_ang_cdf.pdf}\label{fig:case141_sim03_bus_volterr_ang_cdf}}
    %
    \caption{(a) Average RMSE for estimated voltage angle at unobserved buses vs. sample size which is the total number of buses and lines with observed state data.
    The circles represent where (b) is located in (a).
    (b) Cumulative Distribution Function of voltage angle estimation error at unmeasured buses given 140 bus/line measurement samples.}
\end{figure}


\subsubsection{Results}

%%%% Calculations
Because all other state quantities can be derived from the complex bus voltages and the physical properties of the power system equipment, our focus in these simulations is on the accuracy of the estimated complex voltages at the buses.
The estimated voltage angle is calculated by translating $\text{Re}(V_s)$ and $\text{Im}(V_s)$ from the estimated state matrix into polar form.
The estimated voltage magnitude $|V_s|$ is taken directly from the estimated state matrix.
The error is calculated by subtracting the estimation from the true value and are only of the unobserved matrix elements.

%%%% Error vs. Sample size
Figures \ref{fig:case141_sim03_bus_volterr_mag_vs_samp} and \ref{fig:case141_sim03_bus_volterr_angle_vs_samp} respectively give the average estimation error of the voltage magnitude and voltage angle versus the sample size.
The average error is calculated as the RMSE for each random sampling averaged over all the samplings, and the sample size refers to the number of observed buses and lines.
In all cases, the added constraints give lower error than not using any constraints.
For small and medium sample sizes, using the power system equations that are linear with the linear approximation equations gives the best accuracy.
But at high sample sizes, the best accuracy comes from using only power system equations that are linear.
This is because the linear approximation equations \eqref{eq:lin_approx_const} are not satisfied exactly in the underlying state matrix $\mathbf{M}$ but instead could be satisfied with an added small error term.
Since they approximately relate complex power flows to voltage magnitudes, even alone they can greatly reduce estimation error with little samples (See ``w/ appx" in Figure \ref{fig:case141_sim03_bus_volterr_mag_vs_samp}).
However with more samples, the added error from their linear approximation affects the estimation of the other quantities which can be seen in the voltage angles (See ``w/ const+appx" vs. ``w/ const" in Figure \ref{fig:case141_sim03_bus_volterr_angle_vs_samp}).

%%%% CDF
To investigate deeper into the estimation error at a specific sample size, the estimation error Cumulative Distribution Functions (CDFs) for voltage magnitude and voltage angle are plotted in Figures \ref{fig:case141_sim03_bus_volterr_mag_cdf} and \ref{fig:case141_sim03_bus_volterr_ang_cdf}, respectively.
The sample size of 140 was chosen to represent 50\% of the buses and lines being observed which has its location marked in Figures \ref{fig:case141_sim03_bus_volterr_mag_vs_samp} and \ref{fig:case141_sim03_bus_volterr_angle_vs_samp} by circles.
Recall that when a bus or line is sampled, only about half of the elements in its row are measured.
The linear approximation equations that relate complex power flows to voltage magnitudes help make the estimation error of the voltage magnitude tightly concentrate around zero.
However without the approximation equations, the voltage magnitude estimation will be exactly correct with a little less than 18\% probability but will be severely under-estimated when wrong.
On the other hand for the voltage angle estimation, most of the accuracy comes from the power system equations that are linear and are slightly improved by the approximation equations.
In all cases, the voltage angles tend to be over-estimated.




%\begin{figure}
%    \includegraphics[width=0.95\columnwidth]{images/case33_sim01_prob_vs_samp.pdf}
%    \caption{Probability of exact matrix completion vs. sample size.
%    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints and solving it without constraints.}
%    \label{fig:case33_sim01_prob_vs_samp}
%\end{figure}

%\hl{\textbf{Use Power System emulator to generate distribution network state data (under different situations).}}

%\hl{\textbf{Add error to measurements (Change problem into Matrix Completion with Error Formulation?).}}


%\hl{\textbf{Estimate at different sample sizes and compare against Nuclear Norm Minimization not having constraints.}}

%\hl{\textbf{Compare accuracy of state estimation vs. amount of error added.}}

%\hl{\textbf{Compare true state with respect to our new assumption bound.}}

==> sections/archived_sections/proof_with_a.tex <==
The follow lemmas will be useful in proving the main lemmas that make up Theorem \ref{thm:samp_complex}.

%%%% Concentration bounds of a supremum

\begin{lemma}
    \label{thm:bound_supremum}
    \fixes{Let $Y_1,\dots,Y_n$ be a sequence of independent random variables from a Banach space, and let $\mathcal{F}$ be a countable family of real valued functions such that if $f\in\mathcal{F}$ then $-f\in\mathcal{F}$.
    Define a specific value resulting from the sequence as
    \begin{align}
        Y_\text{sup}:= \sup_{f\in\mathcal{F}} \sum_{i=1}^n f(Y_i). \nonumber
    \end{align}
    If $|f|\leq B$ for positive constant $B$ and $\mathbb{E}(f(Y_i))=0$ for all $f\in\mathcal{F}$ and $i\in\{1,\dots,n\}$, then for any $t\geq 0$
    \begin{align}
        \mathbb{P}(|Y_\text{sup}-\mathbb{E}(Y_\text{sup})| > t) \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber \\ \leq 3 \exp\left(-\frac{t}{KB}\log\left(1+\frac{Bt}{\sigma^2+B\mathbb{E}(Y_\text{sup})}\right)\right) \nonumber
    \end{align}
    where $K$ is a numerical constant and $\sigma^2:=\sup_{f\in\mathcal{F}} \sum_{i=1}^n \mathbb{E}((f(Y_i))^2)$.}
\end{lemma}

\fixes{The proof can be found in \cite{talagrand1996new}.}

%%%% Bound on expectation of Z

\begin{lemma}
    \label{thm:bound_expectation}
    \fixes{There exists a constant $C'_R$ such that
    \begin{align}
        \mathbb{E}\left(\frac{1}{p}\left\|\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega-p\mathbf{I}\right)\mathcal{P}_\mathcal{T}\right\|\right) \leq C'_R \sqrt{\frac{\mu_0 r n_1 \log n_1}{m}} \nonumber
    \end{align} as long as the RHS is smaller than 1.}
\end{lemma}

\fixes{The proof can be found in \cite{candes2007sparsity}.}

%%%% Bound the operator norm of H

\begin{lemma}
    \label{thm:bound_opnormH}
    Suppose that if $\Omega$ is sampled according to the Bernoulli model \eqref{eq:bernoulli}, $n_1\geq n_2$, and Assumption \ref{ass:coherence} is satisfied, then there is a numerical constant $C_R$ such that for all $\beta>1$,
    \begin{align}
        \frac{1}{p\fixes{+q}}\left\|\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega\fixes{+a\mathcal{P}_\mathcal{Q}}\right)\mathcal{P}_\mathcal{T}-(p\fixes{+q})\mathcal{P}_\mathcal{T}\right\| \quad\quad\quad \quad\quad\quad \nonumber \\
        \leq \frac{C_R \sqrt{\mu_0\beta rn_1\log n_1}\fixes{+n_1n_2\sqrt{C_{\mathcal{Q}1}(q,a)}}}{\sqrt{m\fixes{+qn_1n_2}}} \nonumber
    \end{align}
    with probability at least $1-3n_1^{-\beta}$ provided that $C_R \sqrt{\frac{\mu_0\beta rn_1\log n_1}{m\fixes{+qn_1n_2}}}<1$ \fixes{and $C_{\mathcal{Q}1}(q,a)\frac{n_1^2n_2^2}{m+qn_1n_2}\leq 1$, where
    \begin{align}
        C_{\mathcal{Q}1}(q,a):=a\mu_\mathcal{Q}+q\left(\left(\sqrt{\mu_\mathcal{Q}}+\sqrt{\mu_{\mathcal{Q}^\perp}}\right)^2-2\mu_\mathcal{Q}\right). \nonumber
    \end{align}}
\end{lemma}

\begin{proof}
    \fixes{First, by the triangle inequality we have
    \begin{align}
        \frac{1}{p+q}\left\|\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega+a\mathcal{P}_\mathcal{Q}\right)\mathcal{P}_\mathcal{T}-(p+q)\mathcal{P}_\mathcal{T}\right\| \quad\quad\quad \quad\quad\quad \nonumber \\
        \leq \frac{1}{p+q}\left(\left\|\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega-p\mathbf{I}\right)\mathcal{P}_\mathcal{T}\right\| + \left\|\mathcal{P}_\mathcal{T}\left(a\mathcal{P}_\mathcal{Q}-q\mathbf{I}\right)\mathcal{P}_\mathcal{T}\right\|\right) \label{eq:Hnorm_2terms}
    \end{align}
    and will analyze each term independently.}

    \fixes{Any matrix $\mathbf{X}\in\mathbb{R}^{n_1\times n_2}$ can be written as
    \begin{align}
        \mathbf{X}=\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathbf{X},\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathbf{e}_i\mathbf{e}_j^\intercal. \nonumber
    \end{align}
    Then step-by-step, we form the inside of the first term
    \begin{align}
        \mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega-p\mathbf{I}\right)\mathcal{P}_\mathcal{T}(\mathbf{X}) \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber
    \end{align}
    \begin{align}
        & =\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega-p\mathbf{I}\right)\mathcal{P}_\mathcal{T}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathbf{X},\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathbf{e}_i\mathbf{e}_j^\intercal \nonumber \\
        & =\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega-p\mathbf{I}\right)\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathcal{P}_\mathcal{T}(\mathbf{X}),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathbf{e}_i\mathbf{e}_j^\intercal \nonumber \\
        & =\mathcal{P}_\mathcal{T}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}(\delta_{ij}-p)\langle \mathcal{P}_\mathcal{T}(\mathbf{X}),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathbf{e}_i\mathbf{e}_j^\intercal \nonumber \\
        & =\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}(\delta_{ij}-p)\langle \mathcal{P}_\mathcal{T}(\mathbf{X}),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) \nonumber \\
        & =\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}(\delta_{ij}-p)\langle \mathbf{X},\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) \rangle \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) \label{eq:Hnorm_2terms1}
    \end{align}
    and likewise, form the inside of the second term
    \begin{align}
        \mathcal{P}_\mathcal{T}\left(a\mathcal{P}_\mathcal{Q}-q\mathbf{I}\right)\mathcal{P}_\mathcal{T}(\mathbf{X}) \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber
    \end{align}
    \begin{align}
        & = \mathcal{P}_\mathcal{T}\left(a\mathcal{P}_\mathcal{Q}-q\mathbf{I}\right)\mathcal{P}_\mathcal{T}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathbf{X},\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathbf{e}_i\mathbf{e}_j^\intercal \nonumber \\
        & = a\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{T}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathbf{X},\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathbf{e}_i\mathbf{e}_j^\intercal \nonumber \\
        & \quad\quad - q\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{T}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathbf{X},\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathbf{e}_i\mathbf{e}_j^\intercal \nonumber \\
        & = a\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{T}(\mathbf{X}),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathbf{e}_i\mathbf{e}_j^\intercal \nonumber \\
        & \quad\quad - q\mathcal{P}_\mathcal{T}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathcal{P}_\mathcal{T}(\mathbf{X}),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathbf{e}_i\mathbf{e}_j^\intercal \nonumber \\
        & = a\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathcal{P}_\mathcal{Q}\mathcal{P}_\mathcal{T}(\mathbf{X}),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal) \nonumber \\
        & \quad\quad - q\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathcal{P}_\mathcal{T}(\mathbf{X}),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) \nonumber \\
        & = a\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathbf{X},\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal) \rangle \mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal) \nonumber \\
        & \quad\quad - q\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathbf{X},\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) \rangle \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal). \label{eq:Hnorm_2terms2}
    \end{align}
    Both terms in \eqref{eq:Hnorm_2terms} will be analyzed separately using \eqref{eq:Hnorm_2terms1} and \eqref{eq:Hnorm_2terms2}, and then applied back together for the lemma's statement.}
    
    \fixes{Before analyzing them, from \eqref{eq:PT_defn} we have that
    \begin{align}
        \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) & = \mathbf{P}_\mathcal{U}(\mathbf{e}_i\mathbf{e}_j^\intercal) + (\mathbf{e}_i\mathbf{e}_j^\intercal)\mathbf{P}_\mathcal{V} - \mathbf{P}_\mathcal{U}(\mathbf{e}_i\mathbf{e}_j^\intercal)\mathbf{P}_\mathcal{V} \nonumber \\
        & = (\mathbf{P}_\mathcal{U}\mathbf{e}_i)\mathbf{e}_j^\intercal + \mathbf{e}_i(\mathbf{P}_\mathcal{V}\mathbf{e}_j)^\intercal - (\mathbf{P}_\mathcal{U}\mathbf{e}_i)(\mathbf{P}_\mathcal{V}\mathbf{e}_j)^\intercal \nonumber
    \end{align}
    which allows for the following upper bound on its Frobenius norm
    \begin{align}
        \|\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\|_F^2 & = \langle \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal),\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) \rangle \nonumber \\
        & = \langle \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \nonumber \\
        & = \langle (\mathbf{P}_\mathcal{U}\mathbf{e}_i)\mathbf{e}_j^\intercal,\mathbf{e}_i\mathbf{e}_j^\intercal \rangle + \langle \mathbf{e}_i(\mathbf{P}_\mathcal{V}\mathbf{e}_j)^\intercal,\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \nonumber \\
        & \quad\quad - \langle (\mathbf{P}_\mathcal{U}\mathbf{e}_i)(\mathbf{P}_\mathcal{V}\mathbf{e}_j)^\intercal,\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \nonumber \\
        & = \langle (\mathbf{P}_\mathcal{U}\mathbf{e}_i),\mathbf{e}_i\mathbf{e}_j^\intercal\mathbf{e}_j \rangle + \langle  {e}_j^\intercal,(\mathbf{P}_\mathcal{V}\mathbf{e}_j)\mathbf{e}_i^\intercal\mathbf{e}_i \rangle \nonumber \\
        & \quad\quad - \langle (\mathbf{P}_\mathcal{U}\mathbf{e}_i)(\mathbf{P}_\mathcal{V}\mathbf{e}_j)^\intercal,\mathbf{P}_\mathcal{U}\mathbf{e}_i\mathbf{e}_j^\intercal \rangle \nonumber \\
        & = \langle (\mathbf{P}_\mathcal{U}\mathbf{e}_i),\mathbf{e}_i \rangle + \langle  {e}_j^\intercal,(\mathbf{P}_\mathcal{V}\mathbf{e}_j) \rangle \nonumber \\
        & \quad\quad - \langle \mathbf{e}_j,(\mathbf{P}_\mathcal{V}\mathbf{e}_j)(\mathbf{P}_\mathcal{U}\mathbf{e}_i)^\intercal(\mathbf{P}_\mathcal{U}\mathbf{e}_i) \rangle \nonumber \\
        & = \langle (\mathbf{P}_\mathcal{U}\mathbf{e}_i),(\mathbf{P}_\mathcal{U}\mathbf{e}_i) \rangle + \langle  (\mathbf{P}_\mathcal{V}\mathbf{e}_j),(\mathbf{P}_\mathcal{V}\mathbf{e}_j) \rangle \nonumber \\
        & \quad\quad - \|\mathbf{P}_\mathcal{U}\mathbf{e}_i\|_F^2\langle \mathbf{e}_j,(\mathbf{P}_\mathcal{V}\mathbf{e}_j) \rangle \nonumber \\
        & = \|\mathbf{P}_\mathcal{U}\mathbf{e}_i\|_F^2 + \|\mathbf{P}_\mathcal{V}\mathbf{e}_j\|_F^2 \nonumber \\
        & \quad\quad - \|\mathbf{P}_\mathcal{U}\mathbf{e}_i\|_F^2\langle (\mathbf{P}_\mathcal{V}\mathbf{e}_j),(\mathbf{P}_\mathcal{V}\mathbf{e}_j) \rangle \nonumber \\
        & = \|\mathbf{P}_\mathcal{U}\mathbf{e}_i\|_F^2 + \|\mathbf{P}_\mathcal{V}\mathbf{e}_j\|_F^2 - \|\mathbf{P}_\mathcal{U}\mathbf{e}_i\|_F^2 \|\mathbf{P}_\mathcal{V}\mathbf{e}_j\|_F^2 \nonumber \\
        & \leq \|\mathbf{P}_\mathcal{U}\mathbf{e}_i\|_F^2 + \|\mathbf{P}_\mathcal{V}\mathbf{e}_j\|_F^2 \nonumber \\
        & \leq \frac{\mu(\mathcal{U})r}{n_1}  + \frac{\mu(\mathcal{V})r}{n_2} \leq 2\frac{\mu_0r}{n_2} \label{eq:PTeiej_mu0}
    \end{align}
    where the fourth and fifth equalities come from applying the cyclic property of the trace operator.}
    
    \fixes{Bounding the first term of \eqref{eq:Hnorm_2terms} at high probability will come from the application of Lemma \ref{thm:bound_supremum} where $Y_{ij}:=\delta_{ij}-p$ and $f(Y_{ij}):=\frac{1}{p+q}Y_{ij}\langle \mathbf{X}_1,\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) \rangle \langle \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal), \mathbf{X}_2 \rangle$ for some $\mathbf{X}_1:\|\mathbf{X}_1\|_F\leq 1$ and $\mathbf{X}_2:\|\mathbf{X}_2\|_F\leq 1$.
    At this point, the condition $\mathbb{E}(f(Y_{ij}))=0$ is already satisfied.
    We can rewrite the first term of \eqref{eq:Hnorm_2terms} with \eqref{eq:Hnorm_2terms1} as
    \begin{align}
        \frac{1}{p+q}\left\|\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega-p\mathbf{I}\right)\mathcal{P}_\mathcal{T}\right\| \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber
    \end{align}
    \begin{align}
         & =\sup \frac{\left\langle \mathbf{X}_1, \sum_{i=1}^{n_1}\sum_{j=1}^{n_2}(\delta_{ij}-p)\langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) \right\rangle}{p+q}  \nonumber \\
         & =\sup \sum_{i=1}^{n_1}\sum_{j=1}^{n_2} \frac{(\delta_{ij}-p)}{p+q}  \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \nonumber \\
         & =: Y_\text{sup} \nonumber
    \end{align}
    where the supremum is on $\mathbf{X}_1:\|\mathbf{X}_1\|_F\leq 1$ and $\mathbf{X}_2:\|\mathbf{X}_2\|_F\leq 1$.
    To determine $B$, we have
    \begin{align}
        |f(\delta_{ij}-p)| & = \frac{|\delta_{ij}-p|}{p+q} |\langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| |\langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| \nonumber \\
        & \leq \frac{|\delta_{ij}-p|}{p+q} \|\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\|_F^2 \|\mathbf{X}_1\|_F \|\mathbf{X}_1\|_F \nonumber \\
        & \leq \frac{|\delta_{ij}-p|}{p+q} \|\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\|_F^2 \nonumber \\
        & \leq \frac{1}{p+q} \|\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\|_F^2 \nonumber \\
        & \leq \frac{2r\mu_0}{(p+q)n_2} \nonumber \\
        & = \frac{2r\mu_0n_1}{m+qn_1n_2} =: B \nonumber
    \end{align}
    where the fourth inequality comes from applying \eqref{eq:PTeiej_mu0} and the last equality is from $p=\frac{m}{n_1n_2}$.
    Lastly, $\sigma^2$ needs to be determined.
    Note that second moment of $(\delta_{ij}-p)$ is $\mathbb{E}((\delta_{ij}-p)^2) = \mathbb{E}(\delta_{ij}^2-2\delta_{ij}+p^2) = p(1-p)$.
    The summand inside the definition of $\sigma^2$ is
    \begin{align}
        \mathbb{E}((f(\delta_{ij}-p))^2) \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber
    \end{align}
    \begin{align}
        & = \frac{\mathbb{E}((\delta_{ij}-p)^2)}{(p+q)^2} \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle^2 \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle^2 \nonumber \\
        & = \frac{p(1-p)}{(p+q)^2} \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle^2 \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle^2 \nonumber \\
        & = \frac{p(1-p)}{(p+q)^2} \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle^2 \langle \mathcal{P}_\mathcal{T}(\mathbf{X}_2),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle^2 \nonumber \\
        & \leq \frac{p(1-p)}{(p+q)^2} \|\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\|_F^2 \|\mathbf{X}_1\|_F^2 \langle \mathcal{P}_\mathcal{T}(\mathbf{X}_2),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle^2 \nonumber \\
        & \leq \frac{p(1-p)}{(p+q)^2} \|\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\|_F^2 \langle \mathcal{P}_\mathcal{T}(\mathbf{X}_2),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle^2 \nonumber \\
        & \leq \frac{p}{(p+q)^2} \|\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\|_F^2 \langle \mathcal{P}_\mathcal{T}(\mathbf{X}_2),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle^2 \nonumber \\
        & \leq \frac{2r\mu_0}{n_2}\frac{p}{(p+q)^2} \langle \mathcal{P}_\mathcal{T}(\mathbf{X}_2),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle^2 \nonumber \\
        & \leq \frac{2r\mu_0}{n_2}\frac{1}{p+q} \langle \mathcal{P}_\mathcal{T}(\mathbf{X}_2),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle^2 \nonumber \\
        & = \frac{2r\mu_0n_1}{m+qn_1n_2} \langle \mathcal{P}_\mathcal{T}(\mathbf{X}_2),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle^2 \nonumber
    \end{align}
    where the fourth inequality comes from applying \eqref{eq:PTeiej_mu0}.
    To determine an upper bound on $\sigma^2$ we have
    \begin{align}
        \sigma^2 & = \sup \sum_{i=1}^{n_1}\sum_{j=1}^{n_2} \mathbb{E}((f(\delta_{ij}-p))^2) \nonumber \\
        & \leq \sup \frac{2r\mu_0n_1}{m+qn_1n_2}\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathcal{P}_\mathcal{T}(\mathbf{X}_2),\mathbf{e}_i\mathbf{e}_j^\intercal \rangle^2 \nonumber \\
        & = \sup \frac{2r\mu_0n_1}{m+qn_1n_2}\|\mathcal{P}_\mathcal{T}(\mathbf{X}_2)\|_F^2 \nonumber \\
        & \leq \frac{2r\mu_0n_1}{m+qn_1n_2}. \nonumber
    \end{align}
    From Lemma \ref{thm:bound_expectation} and multiplying it by $\frac{p}{p+q}$, we bound the expectation of the first term of \eqref{eq:Hnorm_2terms} to be less than 1 which also satisfies the condition of Lemma \ref{thm:bound_expectation}
    \begin{align}
        \mathbb{E}\left(\frac{1}{p+q}\left\|\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega-p\mathbf{I}\right)\mathcal{P}_\mathcal{T}\right\|\right) \quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber
    \end{align}
    \begin{align}
        & \leq  C'_R \frac{p}{p+q} \sqrt{\frac{\mu_0 r n_1 \log n_1}{m}} \nonumber \\
        & =  C'_R \frac{m}{m+qn_1n_2} \sqrt{\frac{\mu_0 r n_1 \log n_1}{m}} \nonumber \\
        & =  C'_R \sqrt{\frac{m}{m+qn_1n_2}} \sqrt{\frac{\mu_0 r n_1 \log n_1}{m+qn_1n_2}} \nonumber \\
        & \leq  C'_R \sqrt{\frac{\mu_0 r n_1 \log n_1}{m+qn_1n_2}} \label{eq:Hnorm_2terms1_expecation} \\
        & = \left(C_R-\sqrt{\frac{4K}{\log 2}}\right) \sqrt{\frac{\mu_0 r n_1 \log n_1}{m+qn_1n_2}} \nonumber \\
        & \leq C_R \sqrt{\frac{\mu_0 r n_1 \log n_1}{m+qn_1n_2}} < 1 \nonumber 
    \end{align}
    where the third equality comes from setting $C'_R:=C_R - \sqrt{\frac{4K}{\log 2}}$ which will be used again later and the last line comes from the assumption in the lemma's statement for any $\beta>1$.}
    
    \fixes{Using the above results, we apply Lemma \ref{thm:bound_supremum} to bound the distance the first term of \eqref{eq:Hnorm_2terms} is from its expected value.
    \begin{align}
        \mathbb{P}(|Y_\text{sup}-\mathbb{E}(Y_\text{sup})| > t) \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber
    \end{align}
    \begin{align}
        & \leq 3 \exp\left(-\frac{t}{KB}\log\left(1+\frac{Bt}{\sigma^2+B\mathbb{E}(Y_\text{sup})}\right)\right) \nonumber \\
        & \leq 3 \exp\left(-\frac{t \log 2}{KB}\min\left\{1,\frac{Bt}{\sigma^2+B\mathbb{E}(Y_\text{sup})}\right\}\right) \nonumber \\
        & \leq 3 \exp\left(-\frac{t(m+qn_1n_2) \log 2}{2Kr\mu_0n_1}\min\left\{1,\frac{t}{2}\right\}\right) \nonumber
    \end{align}
    where the second inequality comes from the fact for any $u\geq 0$, we have $\log (1+u)\geq \log 2 \min\{1,u\}$.
    Set $t:=\sqrt{\left(\frac{4K}{\log 2}\right)\frac{\beta r \mu_0 n_1 \log n_1}{m+qn_1n_2}}$ to get the following
    \begin{align}
        \mathbb{P}\left(|Y_\text{sup}-\mathbb{E}(Y_\text{sup})| > \sqrt{\left(\frac{4K}{\log 2}\right)\frac{\beta r \mu_0 n_1 \log n_1}{m+qn_1n_2}}\right) \quad\qaud\quad\qaud \nonumber
    \end{align}
    \begin{align}
        & \leq 3 \exp\left(-\min\left\{\sqrt{\frac{\log 2}{K}\frac{\beta (m+qn_1n_2) \log n_1}{r \mu_0 n_1}},\beta \log n_1\right\}\right) \nonumber \\
        & = 3 n_1^{-\beta} \label{eq:Hnorm_2terms1_concentration}
    \end{align}
    where the equality is sufficiently true when we have $C_R = C'_R + \sqrt{\frac{4K}{\log 2}}$ and assume $C_R \sqrt{\frac{\mu_0\beta rn_1\log n_1}{m\fixes{+qn_1n_2}}}<1$ from the lemma's statement.}
    
    \fixes{Bringing together the bound on the expectation \eqref{eq:Hnorm_2terms1_expecation} and concentration \eqref{eq:Hnorm_2terms1_concentration} of the first term of \eqref{eq:Hnorm_2terms}, we have
    \begin{align}
        \frac{1}{p+q}\left\|\mathcal{P}_\mathcal{T}\left(\mathcal{P}_\Omega-p\mathbf{I}\right)\mathcal{P}_\mathcal{T}\right\| \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber
    \end{align}
    \begin{align}
        & \leq  C'_R \sqrt{\frac{\mu_0 r n_1 \log n_1}{m+qn_1n_2}} + \sqrt{\left(\frac{4K}{\log 2}\right)\frac{\beta r \mu_0 n_1 \log n_1}{m+qn_1n_2}} \nonumber \\ 
        & \leq C_R\sqrt{\frac{\beta r \mu_0 n_1 \log n_1}{m+qn_1n_2}} \label{eq:Hnorm_2terms1_final}
    \end{align}
    with probability $1-3n_1^{-\beta}$ for $\beta>1$ and setting $C_R := C'_R + \sqrt{\frac{4K}{\log 2}}$.}
    
    \fixes{Now we move on to analyze the second term of \eqref{eq:Hnorm_2terms} with \eqref{eq:Hnorm_2terms2}
    \begin{align}
        \frac{1}{p+q}\left\|\mathcal{P}_\mathcal{T}\left(a\mathcal{P}_\mathcal{Q}-q\mathbf{I}\right)\mathcal{P}_\mathcal{T}\right\| \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \nonumber
    \end{align}
    \begin{align}
         & =\sup \frac{\left\langle \mathbf{X}_1, a\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal) \right\rangle}{p+q}  \nonumber \\
         & \quad\qaud -\frac{\left\langle \mathbf{X}_1, q\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal) \right\rangle}{p+q}  \nonumber \\
         & =\sup \frac{1}{p+q} \sum_{i=1}^{n_1}\sum_{j=1}^{n_2} a  \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \nonumber \\
         & \quad - \frac{1}{p+q} \sum_{i=1}^{n_1}\sum_{j=1}^{n_2} q  \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \label{eq:Hnorm_2terms2_expanded}
    \end{align}
    where the supremum is on $\mathbf{X}_1:\|\mathbf{X}_1\|_F\leq 1$ and $\mathbf{X}_2:\|\mathbf{X}_2\|_F\leq 1$.
    Analyzing the inside of the summation for a particular $(i,j)$, we have
    \begin{align}
        & a  \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \quad\quad\quad\quad\quad\quad\quad\quad \nonumber \\
        & \quad -  q  \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \nonumber
    \end{align}
    \begin{align}
        & = (a-q)  \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \nonumber \\
        & \quad - q \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_{\mathcal{Q}^\perp}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_{\mathcal{Q}^\perp}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \nonumber \\
        & \quad - q \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_{\mathcal{Q}^\perp}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \nonumber \\
        & \quad - q \langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_{\mathcal{Q}^\perp}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle \nonumber \\
        & \leq |a-q|  |\langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| |\langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| \nonumber \\
        & \quad + q |\langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_{\mathcal{Q}^\perp}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| |\langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_{\mathcal{Q}^\perp}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| \nonumber \\
        & \quad + q |\langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| |\langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_{\mathcal{Q}^\perp}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| \nonumber \\
        & \quad + q |\langle \mathbf{X}_1, \mathcal{P}_\mathcal{T}\mathcal{P}_{\mathcal{Q}^\perp}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| |\langle \mathbf{X}_2,\mathcal{P}_\mathcal{T}\mathcal{P}_\mathcal{Q}(\mathbf{e}_i\mathbf{e}_j^\intercal)\rangle| \nonumber
    \end{align}
    where the first equality comes from substituting $\mathcal{P}_\mathcal{T}(\mathcal{P}_\mathcal{Q}+\mathcal{P}_{\mathcal{Q}^\perp})(\mathbf{e}_i\mathbf{e}_j^\intercal)=\mathcal{P}_\mathcal{T}(\mathbf{e}_i\mathbf{e}_j^\intercal)$ in the second term.}
\end{proof}

\begin{lemma}
    \label{thm:dualnorm_nuc_spec}
    For each pair $\mathbf{W}$ and $\mathbf{H}$, we have $\langle \mathbf{W},\mathbf{H} \rangle \leq \|\mathbf{W}\| \|\mathbf{H}\|_*$.
    In particular, for each $\mathbf{H}$, there is a $\mathbf{W}$ such that $\|\mathbf{W}\|=1$ where it achieves the equality.
\end{lemma}
This comes directly from the fact that the spectral norm and nuclear norm are dual to each other which is proved in \cite{recht2010guaranteed}.

\subsubsection{Lemma \ref{thm:nuc_norm_opt}}
\label{sec:proof_nuc_norm_opt}

\begin{proof}
    We start by perturbing $\mathbf{X}_0$ by any $\mathbf{H}$ so that $\mathbf{X}_0+\mathbf{H}$ remains feasible to Problem \eqref{eq:nuc_norm_prob}.
    Since $\mathbf{X}_0$ is already feasible, then it must be that $\mathcal{R}_\Omega(\mathbf{H})=\mathbf{0}$ and $\langle \mathbf{A}^{(l)}, \mathbf{H} \rangle = 0$ for all $l\in\{1,\dots,\fixes{h}\}$.
    
    Take any subgradient $\mathbf{Y}^0$ of the nuclear norm at $\mathbf{X}_0$ which also satisfies
    \begin{subequations}
        \begin{align}
            \mathcal{P}_\mathcal{T}(\mathbf{Y}^0) & = \sum_{k=1}^{r}\mathbf{u}_k\mathbf{v}_k^\intercal \\
            \left\|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y}^0)\right\| & \leq 1.
        \end{align}
    \end{subequations}
    Let us also define $\mathbf{W}^0:=\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y}^0)$ and $\mathbf{W}:=\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y})$ for $\mathbf{Y}$ in the lemma's statement.
    This allows us to write $\mathbf{Y}^0=\mathcal{P}_\mathcal{T}(\mathbf{Y}^0)+\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y}^0)=\mathcal{P}_\mathcal{T}(\mathbf{Y}^0)+\mathbf{W}^0$ and $\mathbf{Y}=\mathcal{P}_\mathcal{T}(\mathbf{Y})+\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Y})=\mathcal{P}_\mathcal{T}(\mathbf{Y})+\mathbf{W}$.
    Since $\mathcal{P}_\mathcal{T}(\mathbf{Y}^0)=\mathcal{P}_\mathcal{T}(\mathbf{Y})$, then we have
    \begin{align}
        \mathbf{Y}^0 = \mathbf{W}^0 - \mathbf{W} + \mathbf{Y}. \nonumber
    \end{align}
    
    Starting from the definition of the subgradient we have
    \begin{align}
        \|\mathbf{X}_0+\mathbf{H}\|_* & \geq \|\mathbf{X}_0\|_* + \langle\mathbf{Y}^0,\mathbf{H}\rangle \nonumber \\
        & = \|\mathbf{X}_0\|_* + \langle\mathbf{W}^0 - \mathbf{W} + \mathbf{Y},\mathbf{H}\rangle \nonumber \\
        & = \|\mathbf{X}_0\|_* + \langle\mathbf{W}^0 - \mathbf{W},\mathbf{H}\rangle \nonumber \\
        & \quad + \left\langle \mathcal{R}_\Omega^\intercal\boldsymbol{\lambda}+\sum_{l=1}^{\fixes{h}} \gamma_l\mathbf{A}^{(l)}, \mathbf{H} \right\rangle \nonumber \\
        & = \|\mathbf{X}_0\|_* + \langle\mathbf{W}^0 - \mathbf{W},\mathbf{H}\rangle \nonumber \\
        & \quad + \left\langle \mathcal{R}_\Omega^\intercal\boldsymbol{\lambda}, \mathbf{H} \right\rangle+\sum_{l=1}^{\fixes{h}} \gamma_l\left\langle\mathbf{A}^{(l)}, \mathbf{H} \right\rangle \nonumber \\
        & = \|\mathbf{X}_0\|_* + \langle\mathbf{W}^0 - \mathbf{W},\mathbf{H}\rangle \label{eq:nuc_norm_opt1}
    \end{align}
    The first equality comes from applying the previous equation and the second comes from applying the definition of $\mathbf{Y}$ given in the lemma's statement.
    The last equality comes from the fact that $\mathcal{R}_\Omega(\mathbf{H})=\mathbf{0}$ and $\langle \mathbf{A}^{(l)}, \mathbf{H} \rangle = 0$ for all $l\in\{1,\dots,\fixes{h}\}$.
    
    Let $\mathbf{Z}$ be any matrix that satisfies the following conditions
    \begin{subequations}
        \begin{align}
            \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Z}) & = \mathbf{W}^0 \label{eq:nuc_norm_opt2a} \\
            \|\mathbf{Z}\| & \leq 1 \label{eq:nuc_norm_opt2b} \\
            \langle \mathbf{Z}, \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\rangle & = \|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\|_*. \label{eq:nuc_norm_opt2c}
        \end{align}
    \end{subequations}
    Since $\mathbf{W}^0$ and $\mathbf{W}$ are in $\mathcal{T}^\perp$ and the projection operator is self-adjoint, we have
    \begin{align}
        \langle \mathbf{W}^0 - \mathbf{W}, \mathbf{H}\rangle & = \langle \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{W}^0 - \mathbf{W}), \mathbf{H}\rangle \nonumber \\
        & = \langle \mathbf{W}^0 - \mathbf{W}, \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\rangle \nonumber \\
        & = \langle \mathbf{W}^0, \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\rangle - \langle \mathbf{W}, \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\rangle \nonumber \\
        & \geq \langle \mathbf{W}^0, \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\rangle - \|\mathbf{W}\| \|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\|_* \nonumber \\
        & = \langle \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{Z}), \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\rangle - \|\mathbf{W}\| \|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\|_* \nonumber \\
        & = \langle \mathbf{Z}, \mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\rangle - \|\mathbf{W}\| \|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\|_* \nonumber \\
        & = \|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\|_* - \|\mathbf{W}\| \|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\|_* \label{eq:nuc_norm_opt3}
    \end{align}
    The first inequality applies Lemma \ref{thm:dualnorm_nuc_spec} to the last term.
    The fourth equality applies \eqref{eq:nuc_norm_opt2a} and the last applies \eqref{eq:nuc_norm_opt2c}.
    
    Finally, plugging \eqref{eq:nuc_norm_opt3} into \eqref{eq:nuc_norm_opt1} gives the following
    \begin{align}
        \|\mathbf{X}_0+\mathbf{H}\|_* \geq \|\mathbf{X}_0\|_* + \left(1 - \|\mathbf{W}\|\right)\|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\|_*.
    \end{align}
    Since $\|\mathbf{W}\|<1$ from the lemma's statement, then $\|\mathbf{X}_0+\mathbf{H}\|_* > \|\mathbf{X}_0\|_*$ unless $\|\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})\|_*=0$.
    This results in $\mathcal{P}_{\mathcal{T}^\perp}(\mathbf{H})=\mathbf{0}$ which means that $\mathbf{H}$ is in $\mathcal{T}$.
    Since $\mathcal{R}_\Omega(\mathbf{H})=\mathbf{0}$, then $\mathbf{H}=\mathbf{0}$ by the given injectivity condition \fixes{along with the fact that $\mathbf{0}\in\mathcal{T}$.}
    Therefore, $\|\mathbf{X}_0+\mathbf{H}\|_* > \|\mathbf{X}_0\|_*$ unless $\mathbf{H}=\mathbf{0}$ which makes $\mathbf{X}_0$ the unique optimal feasible solution to Problem \eqref{eq:nuc_norm_prob}.
\end{proof}

\begin{figure*}
    \centering
    \includegraphics[width=0.60\textwidth]{images/diagram_141bus_PMUs.pdf}
    \caption{Diagram of the 141 bus distribution network~\cite{khodr2008maximum}.
    The two buses with PMUs are labeled by blue circles.}
    \label{fig:diagram_141bus_PMUs}
\end{figure*}

\subsubsection{Lemma \ref{thm:bound_Hsum}}
\label{sec:proof_bound_Hsum}

\begin{proof}
    Starting with the LHS of \eqref{eq:spectral_norm_sum}, we have the following
    \begin{align}
        \frac{1}{p}\left\|\left(\mathcal{P}_{\mathcal{T}^\perp}\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}\right)\sum_{k=k_0}^\infty \mathcal{H}^k(\mathbf{F})\right\| & \leq \frac{1}{p}\left\|\left(\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}\right)\sum_{k=k_0}^\infty \mathcal{H}^k(\mathbf{F})\right\| \nonumber \\
        & \leq \frac{1}{p}\left\|\left(\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}\right)\sum_{k=k_0}^\infty \mathcal{H}^k(\mathbf{F})\right\|_F \nonumber \\
        & \leq \sqrt{\frac{3}{2p}}\left\|\left(\mathcal{P}_\mathcal{T}\right)\sum_{k=k_0}^\infty \mathcal{H}^k(\mathbf{F})\right\|_F \nonumber \\
        & = \sqrt{\frac{3n_1n_2}{2m}}\left\|\sum_{k=k_0}^\infty \mathcal{H}^k(\mathbf{F})\right\|_F. \label{eq:bound_Hsum_1}
    \end{align}
    The first inequality comes from the fact that the projection operator is a non-expansive mapping and the second comes from the Frobenius norm being at least as large as the spectral norm.
    The third comes from applying Lemma \ref{thm:bound_frob_OmegaT} which can be applied since the assumption that $m\geq 4C_R^2\mu_0\beta rn_1\log n_1$ is equivalent to $C_R \sqrt{\frac{\mu_0\beta rn_1\log n_1}{m}}\leq\frac{1}{2}$.
    The equality comes from the fact that $\mathcal{H}$ in \eqref{eq:H_defn} is already projected into $\mathcal{T}$ and $p=\frac{m}{n_1n_2}$.
    
    From here, we focus on bounding the Frobenius norm on the RHS of \eqref{eq:bound_Hsum_1}
    \begin{align}
        \left\|\sum_{k=k_0}^\infty \mathcal{H}^k(\mathbf{F})\right\|_F & \leq \sum_{k=k_0}^\infty \left\|\mathcal{H}^k(\mathbf{F})\right\|_F \nonumber \\
        & \leq \left\|\mathbf{F}\right\|_F\sum_{k=k_0}^\infty \|\mathcal{H}\|^k \nonumber \\
        & = \|\mathbf{F}\|_F\frac{\|\mathcal{H}\|^{k_0}}{1-\|\mathcal{H}\|} \nonumber \\
        & \leq 2\|\mathbf{F}\|_F\|\mathcal{H}\|^{k_0} \nonumber \\
        & \leq 2\|\mathbf{F}\|_F \left(\frac{C_R^2\mu_0\beta rn_1\log n_1}{m}\right)^{k_0/2} \nonumber \\
        & \leq 2 \sqrt{\frac{\mu_Ar}{n_1n_2}} \left(\frac{C_R^2\mu_0\beta rn_1\log n_1}{m}\right)^{k_0/2} \label{eq:bound_Hsum_2}
    \end{align}
    The first inequality comes from the triangle inequality.
    The second inequality comes from one of the equivalent definitions of the operator norm under the Frobenius norm.
    The first equality comes from the geometric series as long as $\|\mathcal{H}\|<1$.
    The third inequality is true as long as $\|\mathcal{H}\|\leq\frac{1}{2}$.
    This true since $\frac{1}{2}\geq C_R \sqrt{\frac{\mu_0\beta rn_1\log n_1}{m}}\geq \frac{1}{p}\left\|\mathcal{P}_\mathcal{T}\mathcal{P}_\Omega\mathcal{P}_\mathcal{T}-p\mathcal{P}_\mathcal{T}\right\|=\|\mathcal{H}\|$ from the assumption that $m\geq 4C_R^2\mu_0\beta rn_1\log n_1$ and Lemma \ref{thm:bound_opnormH}.
    The fourth inequality comes from applying Lemma \ref{thm:bound_opnormH} to $\|\mathcal{H}\|$.
    The last inequality comes from the definition of $\mathbf{F}$ in \eqref{eq:F_defn} and Assumption \ref{ass:equality}.
    
    Finally, plugging \eqref{eq:bound_Hsum_2} into \eqref{eq:bound_Hsum_1} gets the resultant with the same probability as Lemmas \ref{thm:bound_opnormH} and \ref{thm:bound_frob_OmegaT}.
\end{proof}

==> sections/archived_sections/to_do_list.tex <==
\begin{enumerate}
    \item \josh{Done.} Motivational example changes (To better motivate the low-rank approximation):
    \begin{itemize}
        \item \josh{Done.} Emphasize that the data comes directly from the test cases.
        \item \josh{Done.} Use the time series data from Yajing for the 123 bus case similarly as the other cases but now can show a distribution (via box and whiskers plots or 95\% confidence intervals) of normalized singular values vs. matrix rank (singular value index).
    \end{itemize}
    \item \josh{Done} Fix the typos and explanation improvements suggested by Yajing.
    \item \josh{Done.} General explanation improvements:
    \begin{itemize}
        \item \josh{Done.} Check what the arXiv paper is comparing to as baselines and how much improvement it found.
        \item \josh{Done.} Make it more clear and emphasize throughout that the arXiv paper has simulations using the Nuclear Norm Minimization Matrix Completion Technique.
        \item \josh{Done.} Make it more clear and emphasize throughout that Least Squares Minimization and other methods need more data than is available, i.e. be fully observable.
        \item \josh{Done.} Soften our claim that the state is low-rank.  Instead, we use the low-rank assumption for theory because the state can be accurately approximated via PCA dimension reduction.  
        \item \josh{Done.} Highlight our improvements and the challenges better and make them more clear throughout.
    \end{itemize}
    \item \josh{Done.} Simulation changes (To compare to existing methods and better connect simulations to the theory):
    \begin{itemize}
        \item \josh{Done.} Add one baseline of Least Squares Minimization to show the high error (and lower probability of completion) under low observablility.  Therefore, we can remove the ``none" and ``w/ appx" cases since the plots will become too crowded and these cases will become only marginally useful in explaining the results.
        %\item Find what the minimum number of well-placed observations is needed for Least Squares to be ``observable" and report that.
        \item \josh{Done.} Replace the Average Error plots (Figures \ref{fig:case141_sim03_bus_volterr_mag_vs_samp} and \ref{fig:case141_sim03_bus_volterr_angle_vs_samp}) with a plot for a particular error threshold that defines completion (How to define this threshold?) and plot Probability of Completion vs. Number of Samples.
        \item \josh{Done.} Replace the CDFs (Figures \ref{fig:case141_sim03_bus_volterr_mag_cdf} and \ref{fig:case141_sim03_bus_volterr_ang_cdf}) under a set number of observations (What is a good number?) with the plot Probability of Completion vs. Error Threshold that defines completion.
        \item \josh{Done.} Vary the number of constraints (randomly chosen) used in ``w/ const+appx" (OR remove sets of constraints like all of Ohm's Law or all of Kirchhoff's Law constraints, etc.) and calculate $\mu_A$. For the same chosen error threshold that defines completion and the same number of observations chosen previously, plot probability of completion vs. $\mu_A$.  Do this for two or three set sample sizes.
        \item \josh{Done.} Explain clearer the connection between the theory and the simulations in other parts of the paper.
    \end{itemize}
    \item Shorten to 6 pages (including the references and appendix) to fit conference length, and make a longer Technical Report version to put online.  Keep a longer version for online.
\end{enumerate}

==> sections/extra_figures.tex <==
\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/case141_sim03_bus_powererr_vs_samp.pdf}
    \caption{Average RMSE for estimated real and reactive power at unmeasured buses vs. sample size.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints, with additional linear approximation constraints, and solving it without constraints.}
    \label{fig:case141_sim03_bus_powererr_vs_samp}
\end{figure}

\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/case141_sim03_line_losserr_vs_samp.pdf}
    \caption{Average RMSE for estimated real and reactive losses at unmeasured lines vs. sample size.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints, with additional linear approximation constraints, and solving it without constraints.}
    \label{fig:case141_sim03_line_losserr_vs_samp}
\end{figure}

\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/case141_sim03_line_pwrfromerr_vs_samp.pdf}
    \caption{Average RMSE for estimated real and reactive power FROM bus at unmeasured lines vs. sample size.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints, with additional linear approximation constraints, and solving it without constraints.}
    \label{fig:case141_sim03_line_pwrfromerr_vs_samp}
\end{figure}

\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/case141_sim03_line_pwrtoerr_vs_samp.pdf}
    \caption{Average RMSE for estimated real and reactive power TO bus at unmeasured lines vs. sample size.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints, with additional linear approximation constraints, and solving it without constraints.}
    \label{fig:case141_sim03_line_pwrtoerr_vs_samp}
\end{figure}

\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/case141_sim03_bus_currerr_vs_samp.pdf}
    \caption{Average RMSE for estimated real, imaginary, and magnitude of current at unmeasured buses vs. sample size.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints, with additional linear approximation constraints, and solving it without constraints.}
    \label{fig:case141_sim03_bus_currerr_vs_samp}
\end{figure}

\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/case141_sim03_line_currerr_vs_samp.pdf}
    \caption{Average RMSE for estimated real, imaginary, and magnitude of current across unmeasured lines vs. sample size.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints, with additional linear approximation constraints, and solving it without constraints.}
    \label{fig:case141_sim03_line_currerr_vs_samp}
\end{figure}

==> sections/perf_evaluation_toy_old.tex <==
\subsection{Matrix Completion with Constraints}
\label{sec:perf_eval_toy}

The goal of this simulation is to observe the impact of the size of \fixes{$\mu_{\mathcal{Q}^\perp}$, and $\nu_{\mathcal{Q}^\perp}$} on the sample complexity through randomly generated matrix completion examples.

\subsubsection{Setup}

%%%% Generating M
The underlying matrix $\mathbf{M}$ was built by first generating an $n_1\times n_2$ matrix with each element sampled independently from a standard normal distribution.
The singular value decomposition of the generated matrix was taken which gives $n_2$ singular values $(\sigma_1,\dots,\sigma_{n_2})$, assuming $n_1\geq n_2$, and their associated basis vectors $(\mathbf{u}_1,\dots,\mathbf{u}_{n_2})$ and $(\mathbf{v}_1,\dots,\mathbf{v}_{n_2})$.
To make the rank of $\mathbf{M}$ to be $r$, $r$ integers are chosen uniformly at random without replacement from 1 to $n_2$ which correspond to the index of the triplet $(\sigma_k,\mathbf{u}_k,\mathbf{v}_k)$.
The chosen triplets and are combined together in \eqref{eq:svd} to get the final $\mathbf{M}$ that is used in the simulation.

%%%% Generating A and b
The equality constraints \eqref{eq:svd_const} are generated in two steps.
First, each matrix $\mathbf{A}^{(l)}$ is made by generating an $n_1\times n_2$ matrix with each element sampled independently from a standard normal distribution.
Afterwards each vector $b^{(l)}$ is determined by evaluating the LHS of \eqref{eq:svd_const}.
There are $n_1n_2$ equality constraints generated by this process.

%%%% Generating the uniform sampling
The uniform sampling was done by taking a random permutation of all the locations for an $n_1\times n_2$ matrix and using the first $m$ locations as the observed samples.
To increase (decrease) number of samples, the next (previous) locations in the permutation were simply added to (subtracted from) the existing observed samples.
Multiple random permutations were tested in parallel so that a sample probably of exact matrix completion could be calculated among them.
The probability of exact matrix completion for a given sample size was calculated as the fraction of random permutation sequences in which the solution to \eqref{eq:nuc_norm_prob} subtracted from $\mathbf{M}$ resulted in a Frobenius norm smaller that a specific tolerance.

%%%% Specifics
The specifics of this simulation were under the following settings: $n_1=40$, $n_2=5$, $r=2$, 100 random permutations, and the maximum tolerance in the Forbenius norm to determine exact completion was set to $10^{-5}$.

\subsubsection{Results}

%%%% Sample size vs. number of constraints
To demonstrate the sample complexity upper bound given by Theorem \ref{thm:samp_complex}, we fixed 
the probability for exact matrix completion for a given set of linear equality constraints to 95\%.
This was done by increasing the sample size until 95 out of the 100 randomly permuted sequences of matrix locations each gave an exact matrix completion.
The final sample size was recorded in top \fixes{third} of Figure \ref{fig:toy_sim02_samp_muA_vs_numconst} for each set of randomly generated constraints.
The constrained nuclear norm minimization matrix completion method \eqref{eq:nuc_norm_prob} was tested against its unconstrained version.
The figure shows that increasing the number of constraints decreases monotonically the number of samples needed to exactly complete a matrix for a given probability.
Interestingly without the constraints, it required a sample size of 190 which is 95\% of the matrix elements.
This shows the performance increase by taking advantage of constraints when they are available.

%%%% \mu_A vs. number of constraints
Additionally, \fixes{the values of $\mu_{\mathcal{Q}^\perp}$ and  $\nu_{\mathcal{Q}^\perp}$}
for a given set of constraints \fixes{were} plotted against the constraint set size in the bottom \fixes{two thirds} of Figure \ref{fig:toy_sim02_samp_muA_vs_numconst}.
This shows that decreasing \fixes{$\mu_{\mathcal{Q}^\perp}$ and $\nu_{\mathcal{Q}^\perp}$} trend with an increasing constraint set size and a decreasing sample size requirement.
\fixes{Notice that $\mu_{\mathcal{Q}^\perp}$ is linear because each added constraint contributes roughly the same amount of information since they are linearly independent.}
%%%% Sample size vs. \nu_Qperp
The data from Figure \ref{fig:toy_sim02_samp_muA_vs_numconst} were re-plotted in Figure \ref{fig:toy_sim02_samp_vs_muA} to show the sample size requirement vs. \fixes{$\nu_{\mathcal{Q}^\perp}$}.
This shows an approximate linear relationship between the sample complexity and \fixes{$\nu_{\mathcal{Q}^\perp}$ until a specific lower threshold around 0.3.
This indicates that when enough of the subgradient at $\mathbf{M}$ is contained in $\mathcal{Q}$, then exact completion is highly probably with few or no samples.}

\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/toy_sim02_samp_muA_vs_numconst_corrected.pdf}
    \caption{(Top) Minimum sample size for exact matrix completion with 95\% probability  vs. number of linear equality constraints.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints and solving it without constraints.
    (Middle) $\mu_{\mathcal{Q}^\perp}$ vs. number of linear equality constraints.
    (Bottom) $\nu_{\mathcal{Q}^\perp}$ vs. number of linear equality constraints.}
    \label{fig:toy_sim02_samp_muA_vs_numconst}
\end{figure}


\begin{figure}
    \includegraphics[width=0.95\columnwidth]{images/toy_sim02_samp_vs_muA_corrected.pdf}
    \caption{Minimum sample size for exact matrix completion with 95\% probability  vs. $\nu_{\mathcal{Q}^\perp}$.
    The comparison is between solving \eqref{eq:nuc_norm_prob} with equality constraints and solving it without constraints.}
    \label{fig:toy_sim02_samp_vs_muA}
\end{figure}

==> sections/to_do_list_final.tex <==
\subsection{Reviewer's Suggestions}

\begin{enumerate}
    \item \textbf{Reviewer \#1:} No suggestions
    \item \textbf{Reviewer \#2:} The paper is very well written but is a bit ambitious in its scope. The description of the power system model is a bit too long, particularly if we take into account that the linearized form is ultimately used, and the description of the basic matrix completion results seem unnecessarily long. The first half of the paper feels almost like a tutorial paper crammed in a conference format. This in turn limits the amount of interesting discussion that the authors can provide of their results. The notion of coherence for the linear equalities is interesting but I would have liked to have some analytical insight about how they behave with different topologies, sampling structure, or system parameters in general. I would reduce Sections I and II and shift the emphasis of the paper to the description of the main result in Section III. I understand that the journal version provides a more detailed description of the result but it would be interesting to provide more insight and analytical discussion as to how the application to distribution systems impacts the performance.
\end{enumerate}

\subsection{To Do List}
\begin{enumerate}
    \item Theory Corrections
    \begin{enumerate}
        \item \josh{Done.} New definitions: $\nu_0$, $\mathcal{Q}$, $\mu_{\mathcal{Q}^\bot}$, $\nu_{\mathcal{Q}^\bot}$.
        \item \josh{Done.} Statement and Proof of Lemma \ref{thm:nuc_norm_opt}.
        \item \josh{Done.} Statement and Proof of Lemma \ref{thm:bound_opnormH}.
        \item \josh{Done.} Statement and Proof of Lemma \ref{thm:inverse_condition}.
        \item \josh{Done.} Statement and Proof of Lemma \ref{thm:bound_Hsum}.
        \item \josh{Done.} Statement and Proof of Lemma \ref{thm:bound_H0}.
        \item \josh{Done.} Statement and Proof of Theorem \ref{thm:samp_complex}.
        \item \josh{Done.} Final structure Corollaries containing the extreme cases with explanations of the general theorem and specific extreme cases (with $q$).
        \item \josh{Done.} Non-trivial case as a corollary and explanation.
    \end{enumerate}
    \item \josh{Done.} Toy Example Corrections
    \item \josh{Done.} Distribution Network Corrections
    \item \josh{Done.} Acknowledgements Section and Author List.  What are the grants you want listed?
    \item Toy example to verify to ourselves the different cases.
    \item All other co-authors check the proof.
    \item Who will register for the conference? (Required for final paper submission.)
\end{enumerate}
